Resolved Depletion Zones and Spatial Differentiation of N2H+ and N2D+

We present a study on the spatial distribution of N2D+ and N2H+ in thirteen protostellar systems. Eight of thirteen objects observed with the IRAM 30m telescope show relative offsets between the peak N2D+ (J=2-1) and N2H+ (J=1-0) emission. We highlight the case of L1157 using interferometric observations from the Submillimeter Array and Plateau de Bure Interferometer of the N2D+ (J=3-2) and N2H+ (J=1-0) transitions respectively. Depletion of N2D+ in L1157 is clearly observed inside a radius of ~2000 AU (7") and the N2H+ emission is resolved into two peaks at radii of ~1000 AU (3.5"), inside the depletion region of N2D+. Chemical models predict a depletion zone in N2H+ and N2D+ due to destruction of H2D+ at T ~ 20 K and the evaporation of CO off dust grains at the same temperature. However, the abundance offsets of 1000 AU between the two species are not reproduced by chemical models, including a model that follows the infall of the protostellar envelope. The average abundance ratios of N2D+ to N2H+ have been shown to decrease as protostars evolve by Emprechtinger et al., but this is the first time depletion zones of N2D+ have been spatially resolved. We suggest that the difference in depletion zone radii for N2H+ and N2D+ is caused by either the CO evaporation temperature being above 20 K or an H2 ortho-to-para ratio gradient in the inner envelope.

==> tab6.tex <==
\begin{deluxetable}{llc}

\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Source Properties}
\tablehead{
  \colhead{Source}  & \colhead{Distance} & \colhead{N2H+/N2D+ offset} \\
                    & \colhead{(pc)}     & \colhead{($^{\prime\prime}$)} \\

}
\startdata
IRAS 03282+3035  & 230   & 8   \\
HH211-mm         & 230    & 20\tablenotemark{\dagger}  \\
IRAS 04325+2402  & 140    & 0  \\
L1527            & 140    & 35  \\
L1521F           & 140    & 0   \\
RNO43            & 460    & 16  \\
HH108 IRS         & 300    & 0\tablenotemark{a}   \\
HH108 MMS         & 300    & 0   \\
L483             & 200    & 16  \\
L673-SMM2        & 300    & 18  \\
L1152            & 300    & 0\tablenotemark{a}  \\
L1157            & 300    & 5 \\
L1165            & 300    & 8  \\

\enddata
\tablecomments{} 
\tablenotetext{\dagger}{Taken from the column density maps, emission maps are spatially coincident.}
\tablenotetext{a}{Shift between protostar and \nthp\ is observed even though \nthp\ and \ntdp\ are spatially coincident.}
\end{deluxetable}

